Physics-Informed Learning of Characteristic Trajectories for Smoke Reconstruction

We delve into the physics-informed neural reconstruction of smoke and obstacles through sparse-view RGB videos, tackling challenges arising from limited observation of complex dynamics. Existing physics-informed neural networks often emphasize short-term physics constraints, leaving the proper preservation of long-term conservation less explored. We introduce Neural Characteristic Trajectory Fields, a novel representation utilizing Eulerian neural fields to implicitly model Lagrangian fluid trajectories. This topology-free, auto-differentiable representation facilitates efficient flow map calculations between arbitrary frames as well as efficient velocity extraction via auto-differentiation. Consequently, it enables end-to-end supervision covering long-term conservation and short-term physics priors. Building on the representation, we propose physics-informed trajectory learning and integration into NeRF-based scene reconstruction. We enable advanced obstacle handling through self-supervised scene decomposition and seamless integrated boundary constraints. Our results showcase the ability to overcome challenges like occlusion uncertainty, density-color ambiguity, and static-dynamic entanglements. Code and sample tests are at \url{https://github.com/19reborn/PICT_smoke}.

==> fig/comparison/fig_vel_comp_game.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure*}[tp]
	%
     % \vspace{-12pt}
	\includegraphics[width=1.0\linewidth]{fig/comparison/vel_comp_game_1220.pdf}
    % \vspace{-18pt}
	\caption
	{
 % \footnotesize
		Comparison of the reconstruction of fluid's physical attributes on the Game scene.
	}
	%
	\label{fig:comparison_vel_game}
	% \vspace{-16pt}
	%
\end{figure*}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

==> fig/comparison/fig_vel_comp_scalar.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}[tp]
	%
     % \vspace{-12pt}
	\includegraphics[width=1.\linewidth]{fig/comparison/vel_comp_scalar.pdf}
    % \vspace{-18pt}
	\caption
	{
		Comparison of the reconstruction of fluid's physical attributes on the real captured ScalarFlow dataset.
		}
	%
	\label{fig:comparison_vel_scalar}
	% \vspace{-16pt}
	%
\end{figure}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%

==> tab/tab0_symbol_table.tex <==

\begin{table}[tb!]
\footnotesize
\begin{tabular}{cll}
\toprule[2pt]
Symbol & Type & Definition \\
\hline
$ \mathbf{x}$ & vector & spatial position \\
\hline
$t$ & scalar & time \\
\hline
$\mathbf{\widetilde{x}}$ & function & particle trajectory \\
\hline
$\mathcal{E}$ & network & Trajectory Encoder\\
\hline
$\mathcal{Z}$ & vector & neural trajectory feature \\
\hline
$\mathcal{D}$ & network & Trajectory Decoder\\
\hline
$\mathcal{U}$ & function & velocity field \\

\bottomrule[2pt]
\end{tabular}
\end{table}
